Effect of dot size on exciton binding energy and electron-hole recombination probability in CdSe quantum dots

Exciton binding energy and electron-hole recombination probability are presented as the two important metrics for investigating effect of dot size on electron-hole interaction in CdSe quantum dots. Direct computation of electron-hole recombination probability is challenging because it requires an accurate mathematical description of electron-hole wavefunction in the neighborhood of the electron-hole coalescence point. In this work, we address this challenge by solving the electron-hole Schrodinger equation using the electron-hole explicitly correlated Hartree-Fock (eh-XCHF) method. The calculations were performed for a series of CdSe clusters ranging from $\mathrm{Cd}_{20}\mathrm{Se}_{19}$ to $\mathrm{Cd}_{74608}\mathrm{Se}_{74837}$ that correspond to dot diameter range of 1-20 nm. The calculated exciton binding energies and electron-hole recombination probabilities were found to decrease with increasing dot size. Both of these quantities were found to scale as $D_\mathrm{dot}^{-n}$ with respect to the dot diameter D. One of the key insights from this study is that the electron-hole recombination probability decreases at a much faster rate than the exciton binding energy as a function of dot size. It was found that an increase in the dot size by a factor of 16.1, resulted in a decrease in the exciton binding energy and electron-hole recombination probability by a factor of 14.4 and $5.5\times10^{6}$, respectively.

==> plots/plot_be_comparison <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Thu Jun  6 22:32:29 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -1.4, 1.4, 0.05
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "Log [D\sdot\N/1 nm] "
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Log [E\sBE\N/1 eV]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place normal
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.71, 0.83
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s1 hidden false
@    s1 type xy
@    s1 symbol 2
@    s1 symbol size 1.000000
@    s1 symbol color 1
@    s1 symbol pattern 1
@    s1 symbol fill color 1
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 1
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 1
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "plot_be_comparison"
@    s1 legend  "eh-XCHF method (this work)"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 3
@    s2 symbol size 1.000000
@    s2 symbol color 3
@    s2 symbol pattern 1
@    s2 symbol fill color 3
@    s2 symbol fill pattern 1
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 0
@    s2 line linestyle 1
@    s2 line linewidth 1.0
@    s2 line color 3
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 3
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "plot_be_comparison"
@    s2 legend  "Wang and Zunger"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 4
@    s3 symbol size 1.000000
@    s3 symbol color 4
@    s3 symbol pattern 1
@    s3 symbol fill color 4
@    s3 symbol fill pattern 1
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 0
@    s3 line linestyle 1
@    s3 line linewidth 1.0
@    s3 line color 4
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 4
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "plot_be_comparison"
@    s3 legend  "Kucur et al."
@    s4 hidden false
@    s4 type xy
@    s4 symbol 6
@    s4 symbol size 1.000000
@    s4 symbol color 5
@    s4 symbol pattern 1
@    s4 symbol fill color 5
@    s4 symbol fill pattern 1
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 0
@    s4 line linestyle 1
@    s4 line linewidth 1.0
@    s4 line color 5
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 5
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "plot_be_comparison"
@    s4 legend  "Inamdar et al."
@    s5 hidden false
@    s5 type xy
@    s5 symbol 8
@    s5 symbol size 1.000000
@    s5 symbol color 15
@    s5 symbol pattern 1
@    s5 symbol fill color 15
@    s5 symbol fill pattern 0
@    s5 symbol linewidth 1.0
@    s5 symbol linestyle 1
@    s5 symbol char 65
@    s5 symbol char font 0
@    s5 symbol skip 0
@    s5 line type 0
@    s5 line linestyle 1
@    s5 line linewidth 1.0
@    s5 line color 13
@    s5 line pattern 1
@    s5 baseline type 0
@    s5 baseline off
@    s5 dropline off
@    s5 fill type 0
@    s5 fill rule 0
@    s5 fill color 1
@    s5 fill pattern 1
@    s5 avalue off
@    s5 avalue type 2
@    s5 avalue char size 1.000000
@    s5 avalue font 0
@    s5 avalue color 1
@    s5 avalue rot 0
@    s5 avalue format general
@    s5 avalue prec 3
@    s5 avalue prepend ""
@    s5 avalue append ""
@    s5 avalue offset 0.000000 , 0.000000
@    s5 errorbar on
@    s5 errorbar place both
@    s5 errorbar color 15
@    s5 errorbar pattern 1
@    s5 errorbar size 1.000000
@    s5 errorbar linewidth 1.0
@    s5 errorbar linestyle 1
@    s5 errorbar riser linewidth 1.0
@    s5 errorbar riser linestyle 1
@    s5 errorbar riser clip off
@    s5 errorbar riser clip length 0.100000
@    s5 comment "plot_be_comparison"
@    s5 legend  "Querner et al."
@    s7 hidden false
@    s7 type xy
@    s7 symbol 5
@    s7 symbol size 1.170000
@    s7 symbol color 11
@    s7 symbol pattern 1
@    s7 symbol fill color 11
@    s7 symbol fill pattern 1
@    s7 symbol linewidth 1.0
@    s7 symbol linestyle 1
@    s7 symbol char 80
@    s7 symbol char font 0
@    s7 symbol skip 0
@    s7 line type 0
@    s7 line linestyle 1
@    s7 line linewidth 1.0
@    s7 line color 8
@    s7 line pattern 1
@    s7 baseline type 0
@    s7 baseline off
@    s7 dropline off
@    s7 fill type 0
@    s7 fill rule 0
@    s7 fill color 1
@    s7 fill pattern 1
@    s7 avalue off
@    s7 avalue type 2
@    s7 avalue char size 1.000000
@    s7 avalue font 0
@    s7 avalue color 1
@    s7 avalue rot 0
@    s7 avalue format general
@    s7 avalue prec 3
@    s7 avalue prepend ""
@    s7 avalue append ""
@    s7 avalue offset 0.000000 , 0.000000
@    s7 errorbar on
@    s7 errorbar place both
@    s7 errorbar color 11
@    s7 errorbar pattern 1
@    s7 errorbar size 1.000000
@    s7 errorbar linewidth 1.0
@    s7 errorbar linestyle 1
@    s7 errorbar riser linewidth 1.0
@    s7 errorbar riser linestyle 1
@    s7 errorbar riser clip off
@    s7 errorbar riser clip length 0.100000
@    s7 comment "plot_be_comparison"
@    s7 legend  "Meulenberg et al."
@    s8 hidden false
@    s8 type xy
@    s8 symbol 1
@    s8 symbol size 0.830000
@    s8 symbol color 12
@    s8 symbol pattern 1
@    s8 symbol fill color 12
@    s8 symbol fill pattern 1
@    s8 symbol linewidth 1.0
@    s8 symbol linestyle 1
@    s8 symbol char 65
@    s8 symbol char font 0
@    s8 symbol skip 0
@    s8 line type 0
@    s8 line linestyle 1
@    s8 line linewidth 1.0
@    s8 line color 2
@    s8 line pattern 1
@    s8 baseline type 0
@    s8 baseline off
@    s8 dropline off
@    s8 fill type 0
@    s8 fill rule 0
@    s8 fill color 1
@    s8 fill pattern 1
@    s8 avalue off
@    s8 avalue type 2
@    s8 avalue char size 1.000000
@    s8 avalue font 0
@    s8 avalue color 1
@    s8 avalue rot 0
@    s8 avalue format general
@    s8 avalue prec 3
@    s8 avalue prepend ""
@    s8 avalue append ""
@    s8 avalue offset 0.000000 , 0.000000
@    s8 errorbar on
@    s8 errorbar place both
@    s8 errorbar color 12
@    s8 errorbar pattern 1
@    s8 errorbar size 1.000000
@    s8 errorbar linewidth 1.0
@    s8 errorbar linestyle 1
@    s8 errorbar riser linewidth 1.0
@    s8 errorbar riser linestyle 1
@    s8 errorbar riser clip off
@    s8 errorbar riser clip length 0.100000
@    s8 comment "plot_be_comparison"
@    s8 legend  "Franceschetti and Zunger "
@    s9 hidden false
@    s9 type xy
@    s9 symbol 10
@    s9 symbol size 1.240000
@    s9 symbol color 2
@    s9 symbol pattern 1
@    s9 symbol fill color 2
@    s9 symbol fill pattern 1
@    s9 symbol linewidth 1.0
@    s9 symbol linestyle 1
@    s9 symbol char 65
@    s9 symbol char font 0
@    s9 symbol skip 0
@    s9 line type 0
@    s9 line linestyle 1
@    s9 line linewidth 1.0
@    s9 line color 1
@    s9 line pattern 1
@    s9 baseline type 0
@    s9 baseline off
@    s9 dropline off
@    s9 fill type 0
@    s9 fill rule 0
@    s9 fill color 1
@    s9 fill pattern 1
@    s9 avalue off
@    s9 avalue type 2
@    s9 avalue char size 1.000000
@    s9 avalue font 0
@    s9 avalue color 1
@    s9 avalue rot 0
@    s9 avalue format general
@    s9 avalue prec 3
@    s9 avalue prepend ""
@    s9 avalue append ""
@    s9 avalue offset 0.000000 , 0.000000
@    s9 errorbar on
@    s9 errorbar place both
@    s9 errorbar color 2
@    s9 errorbar pattern 1
@    s9 errorbar size 1.000000
@    s9 errorbar linewidth 1.0
@    s9 errorbar linestyle 1
@    s9 errorbar riser linewidth 1.0
@    s9 errorbar riser linestyle 1
@    s9 errorbar riser clip off
@    s9 errorbar riser clip length 0.100000
@    s9 comment "plot_be_comparison"
@    s9 legend  "Jasieniak et al."
@target G0.S1
@type xy
0.095169351 -0.065826789
0.25285303 -0.22097892
0.44090908 -0.40455406
0.47421626 -0.43714089
0.51587384 -0.47807871
0.57886833 -0.5388967
0.68124124 -0.6386539
0.81954394 -0.77082995
1 -0.9409005
1.1760913 -1.1061959
1.30103 -1.2226912
&
@target G0.S2
@type xy
0.31533964 -0.2663005
0.46735959 -0.42908597
0.58525639 -0.54097561
&
@target G0.S3
@type xy
0.50835152 -0.16401662
0.54048802 -0.21522157
0.56977969 -0.25300171
0.57789431 -0.34005054
&
@target G0.S4
@type xy
0.28730918 -0.18599893
0.37833121 -0.12310007
0.42470805 -0.50431971
0.45687398 -0.3912836
0.48684162 -0.5283607
0.52752202 -0.37343279
0.55049692 -0.49263805
&
@target G0.S5
@type xy
0.47521298 -0.094742871
0.63401966 -0.28715003
&
@target G0.S7
@type xy
0.095203336 -0.004201647
0.44171153 -0.12774697
0.47421687 -0.2243597
0.5789887 -0.56384054
&
@target G0.S8
@type xy
0.25527251 -0.17457388
0.52113808 -0.53165267
0.68663627 -0.73518218
&
@target G0.S9
@type xy
0.095169351 0.003555975
0.25042 -0.12520061
0.44090908 -0.30295715
0.47421626 -0.33568272
0.51587384 -0.37718023
0.57886833 -0.44196296
0.68124124 -0.54724938
0.81954394 -0.69480772
1 -0.89290353
1.1760913 -1.0909309
1.30103 -1.2336826
&


==> plots/plot_be_with_dielec <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Tue Jun  4 13:48:12 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -1.4, 1.4, 0.05
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "Log D\sdot\N (nm)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Log Binding Energy (eV)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place normal
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.7, 0.82
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s1 hidden false
@    s1 type xy
@    s1 symbol 2
@    s1 symbol size 1.000000
@    s1 symbol color 1
@    s1 symbol pattern 1
@    s1 symbol fill color 1
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 1
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 1
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "plot_be_comparison"
@    s1 legend  "XCHF Method"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 3
@    s2 symbol size 1.000000
@    s2 symbol color 3
@    s2 symbol pattern 1
@    s2 symbol fill color 3
@    s2 symbol fill pattern 1
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 0
@    s2 line linestyle 1
@    s2 line linewidth 1.0
@    s2 line color 3
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 3
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "plot_be_comparison"
@    s2 legend  "Wang and Zunger"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 4
@    s3 symbol size 1.000000
@    s3 symbol color 4
@    s3 symbol pattern 1
@    s3 symbol fill color 4
@    s3 symbol fill pattern 1
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 0
@    s3 line linestyle 1
@    s3 line linewidth 1.0
@    s3 line color 4
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 4
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "plot_be_comparison"
@    s3 legend  "Kucur et al."
@    s4 hidden false
@    s4 type xy
@    s4 symbol 6
@    s4 symbol size 1.000000
@    s4 symbol color 5
@    s4 symbol pattern 1
@    s4 symbol fill color 5
@    s4 symbol fill pattern 1
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 0
@    s4 line linestyle 1
@    s4 line linewidth 1.0
@    s4 line color 5
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 5
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "plot_be_comparison"
@    s4 legend  "Inamdar et al."
@    s5 hidden false
@    s5 type xy
@    s5 symbol 8
@    s5 symbol size 1.000000
@    s5 symbol color 15
@    s5 symbol pattern 1
@    s5 symbol fill color 15
@    s5 symbol fill pattern 0
@    s5 symbol linewidth 1.0
@    s5 symbol linestyle 1
@    s5 symbol char 65
@    s5 symbol char font 0
@    s5 symbol skip 0
@    s5 line type 0
@    s5 line linestyle 1
@    s5 line linewidth 1.0
@    s5 line color 13
@    s5 line pattern 1
@    s5 baseline type 0
@    s5 baseline off
@    s5 dropline off
@    s5 fill type 0
@    s5 fill rule 0
@    s5 fill color 1
@    s5 fill pattern 1
@    s5 avalue off
@    s5 avalue type 2
@    s5 avalue char size 1.000000
@    s5 avalue font 0
@    s5 avalue color 1
@    s5 avalue rot 0
@    s5 avalue format general
@    s5 avalue prec 3
@    s5 avalue prepend ""
@    s5 avalue append ""
@    s5 avalue offset 0.000000 , 0.000000
@    s5 errorbar on
@    s5 errorbar place both
@    s5 errorbar color 15
@    s5 errorbar pattern 1
@    s5 errorbar size 1.000000
@    s5 errorbar linewidth 1.0
@    s5 errorbar linestyle 1
@    s5 errorbar riser linewidth 1.0
@    s5 errorbar riser linestyle 1
@    s5 errorbar riser clip off
@    s5 errorbar riser clip length 0.100000
@    s5 comment "plot_be_comparison"
@    s5 legend  "Querner et al."
@    s6 hidden false
@    s6 type xy
@    s6 symbol 10
@    s6 symbol size 1.000000
@    s6 symbol color 12
@    s6 symbol pattern 1
@    s6 symbol fill color 12
@    s6 symbol fill pattern 0
@    s6 symbol linewidth 1.0
@    s6 symbol linestyle 1
@    s6 symbol char 65
@    s6 symbol char font 0
@    s6 symbol skip 0
@    s6 line type 0
@    s6 line linestyle 1
@    s6 line linewidth 1.0
@    s6 line color 11
@    s6 line pattern 1
@    s6 baseline type 0
@    s6 baseline off
@    s6 dropline off
@    s6 fill type 0
@    s6 fill rule 0
@    s6 fill color 1
@    s6 fill pattern 1
@    s6 avalue off
@    s6 avalue type 2
@    s6 avalue char size 1.000000
@    s6 avalue font 0
@    s6 avalue color 1
@    s6 avalue rot 0
@    s6 avalue format general
@    s6 avalue prec 3
@    s6 avalue prepend ""
@    s6 avalue append ""
@    s6 avalue offset 0.000000 , 0.000000
@    s6 errorbar on
@    s6 errorbar place both
@    s6 errorbar color 12
@    s6 errorbar pattern 1
@    s6 errorbar size 1.000000
@    s6 errorbar linewidth 1.0
@    s6 errorbar linestyle 1
@    s6 errorbar riser linewidth 1.0
@    s6 errorbar riser linestyle 1
@    s6 errorbar riser clip off
@    s6 errorbar riser clip length 0.100000
@    s6 comment "plot_be_comparison"
@    s6 legend  "Jasieniak et al. SEPM method "
@    s7 hidden false
@    s7 type xy
@    s7 symbol 5
@    s7 symbol size 1.170000
@    s7 symbol color 11
@    s7 symbol pattern 1
@    s7 symbol fill color 11
@    s7 symbol fill pattern 1
@    s7 symbol linewidth 1.0
@    s7 symbol linestyle 1
@    s7 symbol char 80
@    s7 symbol char font 0
@    s7 symbol skip 0
@    s7 line type 0
@    s7 line linestyle 1
@    s7 line linewidth 1.0
@    s7 line color 8
@    s7 line pattern 1
@    s7 baseline type 0
@    s7 baseline off
@    s7 dropline off
@    s7 fill type 0
@    s7 fill rule 0
@    s7 fill color 1
@    s7 fill pattern 1
@    s7 avalue off
@    s7 avalue type 2
@    s7 avalue char size 1.000000
@    s7 avalue font 0
@    s7 avalue color 1
@    s7 avalue rot 0
@    s7 avalue format general
@    s7 avalue prec 3
@    s7 avalue prepend ""
@    s7 avalue append ""
@    s7 avalue offset 0.000000 , 0.000000
@    s7 errorbar on
@    s7 errorbar place both
@    s7 errorbar color 11
@    s7 errorbar pattern 1
@    s7 errorbar size 1.000000
@    s7 errorbar linewidth 1.0
@    s7 errorbar linestyle 1
@    s7 errorbar riser linewidth 1.0
@    s7 errorbar riser linestyle 1
@    s7 errorbar riser clip off
@    s7 errorbar riser clip length 0.100000
@    s7 comment "plot_be_comparison"
@    s7 legend  "Meulenberg et al."
@    s8 hidden false
@    s8 type xy
@    s8 symbol 1
@    s8 symbol size 0.830000
@    s8 symbol color 2
@    s8 symbol pattern 1
@    s8 symbol fill color 2
@    s8 symbol fill pattern 1
@    s8 symbol linewidth 1.0
@    s8 symbol linestyle 1
@    s8 symbol char 65
@    s8 symbol char font 0
@    s8 symbol skip 0
@    s8 line type 0
@    s8 line linestyle 1
@    s8 line linewidth 1.0
@    s8 line color 2
@    s8 line pattern 1
@    s8 baseline type 0
@    s8 baseline off
@    s8 dropline off
@    s8 fill type 0
@    s8 fill rule 0
@    s8 fill color 1
@    s8 fill pattern 1
@    s8 avalue off
@    s8 avalue type 2
@    s8 avalue char size 1.000000
@    s8 avalue font 0
@    s8 avalue color 1
@    s8 avalue rot 0
@    s8 avalue format general
@    s8 avalue prec 3
@    s8 avalue prepend ""
@    s8 avalue append ""
@    s8 avalue offset 0.000000 , 0.000000
@    s8 errorbar on
@    s8 errorbar place both
@    s8 errorbar color 2
@    s8 errorbar pattern 1
@    s8 errorbar size 1.000000
@    s8 errorbar linewidth 1.0
@    s8 errorbar linestyle 1
@    s8 errorbar riser linewidth 1.0
@    s8 errorbar riser linestyle 1
@    s8 errorbar riser clip off
@    s8 errorbar riser clip length 0.100000
@    s8 comment "plot_be_comparison"
@    s8 legend  "Franceschetti and Zunger "
@target G0.S1
@type xy
0.095169351 -0.065826789
0.25285303 -0.22097892
0.440909082	-0.366630954
0.474216264	-0.408224223
0.515873844	-0.459437537
0.578868329	-0.537185793
0.68124124 -0.6386539
0.81954394 -0.77082995
1 -0.9409005
1.1760913 -1.1061959
1.30103 -1.2226912
&
@target G0.S2
@type xy
0.31533964 -0.2663005
0.46735959 -0.42908597
0.58525639 -0.54097561
&
@target G0.S3
@type xy
0.50835152 -0.16401662
0.54048802 -0.21522157
0.56977969 -0.25300171
0.57789431 -0.34005054
&
@target G0.S4
@type xy
0.28730918 -0.18599893
0.37833121 -0.12310007
0.42470805 -0.50431971
0.45687398 -0.3912836
0.48684162 -0.5283607
0.52752202 -0.37343279
0.55049692 -0.49263805
&
@target G0.S5
@type xy
0.47521298 -0.094742871
0.63401966 -0.28715003
&
@target G0.S6
@type xy
0.26883763 -0.14817743
0.28971245 -0.17485052
0.3164543 -0.19166342
0.33951186 -0.22739815
0.37343615 -0.24644835
0.3870663 -0.25958915
0.42818859 -0.29432869
0.44444782 -0.30909191
0.46495296 -0.33219322
0.50546514 -0.3649719
0.54117821 -0.39133279
0.56153129 -0.36487932
0.58464078 -0.40971671
0.62414725 -0.42895768
0.74629994 -0.52831965
0.80794397 -0.52854693
&
@target G0.S7
@type xy
0.095203336 -0.004201647
0.44171153 -0.12774697
0.47421687 -0.2243597
0.5789887 -0.56384054
&
@target G0.S8
@type xy
0.25527251 -0.17457388
0.52113808 -0.53165267
0.68663627 -0.73518218
&
@target G0.S9 
@type xy 
0.095169351	0.003555975
0.250420002	-0.125200607
0.440909082	-0.302957149
0.474216264	-0.335682717
0.515873844	-0.377180231
0.578868329	-0.441962961
0.681241237	-0.547249383
0.819543936	-0.694807722
1	-0.892903531
1.176091259	-1.090930896
1.301029996	-1.233682583
&


==> plots/plot_comp_ddot <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Thu Jun  6 22:47:55 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -0.2, 21, 1.2
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "D\sdot\N (nm)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Property Ratio (X/X\s0\N)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place normal
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.85, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 0
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 0
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "plot_func_comp"
@    s0 legend  ""
@    s1 hidden false
@    s1 type xy
@    s1 symbol 1
@    s1 symbol size 1.240000
@    s1 symbol color 2
@    s1 symbol pattern 1
@    s1 symbol fill color 2
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 100
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 2
@    s1 line pattern 0
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 2
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "Editor"
@    s1 legend  "P\seh\N"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 0
@    s2 symbol size 1.000000
@    s2 symbol color 1
@    s2 symbol pattern 1
@    s2 symbol fill color 1
@    s2 symbol fill pattern 0
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 1
@    s2 line linewidth 1.0
@    s2 line color 1
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 1
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "plot_comp_func"
@    s2 legend  ""
@    s3 hidden false
@    s3 type xy
@    s3 symbol 2
@    s3 symbol size 1.240000
@    s3 symbol color 1
@    s3 symbol pattern 1
@    s3 symbol fill color 1
@    s3 symbol fill pattern 1
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 1
@    s3 line linestyle 1
@    s3 line linewidth 1.0
@    s3 line color 4
@    s3 line pattern 0
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 1
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "plot_comp_func"
@    s3 legend  "E\sBE\N"
@target G0.S0
@type xy
1.33 0.9874199
1.34 0.9462326
1.35 0.9070506
1.4 0.7375539
1.45 0.6041
1.5 0.4981532
1.55 0.4133932
1.6 0.3450925
1.65 0.2896819
1.7 0.2444424
1.75 0.2072858
1.8 0.1765956
1.85 0.1511114
1.9 0.1298433
1.95 0.1120091
2 0.09698652
2.05 0.08427797
2.1 0.07348296
2.15 0.06427766
2.2 0.05639879
2.25 0.04963132
2.3 0.04379879
2.35 0.03875574
2.4 0.03438179
2.45 0.03057689
2.5 0.02725758
2.55 0.02435395
2.6 0.02180729
2.65 0.01956805
2.7 0.01759434
2.75 0.0158506
2.8 0.01430656
2.85 0.01293637
2.9 0.01171791
2.95 0.01063218
3 0.009662829
3.05 0.008795743
3.1 0.008018713
3.15 0.007321155
3.2 0.006693865
3.25 0.006128828
3.3 0.005619048
3.35 0.005158401
3.4 0.004741524
3.45 0.004363701
3.5 0.004020786
3.55 0.003709122
3.6 0.00342548
3.65 0.003167001
3.7 0.002931154
3.75 0.00271569
3.8 0.00251861
3.85 0.002338134
3.9 0.002172674
3.95 0.002020811
4 0.001881277
4.05 0.001752935
4.1 0.001634765
4.15 0.001525852
4.2 0.001425371
4.25 0.001332581
4.3 0.001246813
4.35 0.001167463
4.4 0.001093985
4.45 0.001025884
4.5 0.0009627139
4.55 0.0009040682
4.6 0.0008495784
4.65 0.0007989095
4.7 0.0007517568
4.75 0.0007078427
4.8 0.000666914
4.85 0.0006287399
4.9 0.0005931093
4.95 0.0005598293
5 0.0005287235
5.05 0.0004996302
5.1 0.000472401
5.15 0.0004469001
5.2 0.0004230026
5.25 0.0004005935
5.3 0.0003795674
5.35 0.000359827
5.4 0.0003412827
5.45 0.0003238521
5.5 0.0003074589
5.55 0.0002920327
5.6 0.0002775086
5.65 0.0002638265
5.7 0.0002509307
5.75 0.0002387697
5.8 0.0002272959
5.85 0.0002164649
5.9 0.0002062357
5.95 0.0001965701
6 0.0001874328
6.05 0.0001787909
6.1 0.0001706137
6.15 0.0001628727
6.2 0.0001555414
6.25 0.0001485951
6.3 0.0001420107
6.35 0.0001357666
6.4 0.0001298429
6.45 0.0001242208
6.5 0.0001188827
6.55 0.0001138124
6.6 0.0001089944
6.65 0.0001044144
6.7 0.0001000591
6.75 9.59158e-05
6.8 9.197278e-05
6.85 8.821898e-05
6.9 8.464404e-05
6.95 8.123823e-05
7 7.799241e-05
7.05 7.489801e-05
7.1 7.194697e-05
7.15 6.91317e-05
7.2 6.644507e-05
7.25 6.388037e-05
7.3 6.143128e-05
7.35 5.909185e-05
7.4 5.685648e-05
7.45 5.471988e-05
7.5 5.267706e-05
7.55 5.072333e-05
7.6 4.885424e-05
7.65 4.706562e-05
7.7 4.535349e-05
7.75 4.371414e-05
7.8 4.214401e-05
7.85 4.063978e-05
7.9 3.919829e-05
7.95 3.781654e-05
8 3.649171e-05
8.05 3.522111e-05
8.1 3.400222e-05
8.15 3.283262e-05
8.2 3.171004e-05
8.25 3.063232e-05
8.3 2.959742e-05
8.35 2.860338e-05
8.4 2.764836e-05
8.45 2.673062e-05
8.5 2.584849e-05
8.55 2.500039e-05
8.6 2.418482e-05
8.65 2.340035e-05
8.7 2.264563e-05
8.75 2.191938e-05
8.8 2.122035e-05
8.85 2.054739e-05
8.9 1.989938e-05
8.95 1.927527e-05
9 1.867405e-05
9.05 1.809476e-05
9.1 1.753649e-05
9.15 1.699835e-05
9.2 1.647953e-05
9.25 1.597923e-05
9.3 1.549669e-05
9.35 1.50312e-05
9.4 1.458206e-05
9.45 1.414861e-05
9.5 1.373024e-05
9.55 1.332634e-05
9.6 1.293633e-05
9.65 1.255968e-05
9.7 1.219586e-05
9.75 1.184436e-05
9.8 1.150472e-05
9.85 1.117647e-05
9.9 1.085918e-05
9.95 1.055243e-05
10 1.025581e-05
10.05 9.968951e-06
10.1 9.691478e-06
10.15 9.423043e-06
10.2 9.163307e-06
10.25 8.911948e-06
10.3 8.668658e-06
10.35 8.43314e-06
10.4 8.205109e-06
10.45 7.984294e-06
10.5 7.770434e-06
10.55 7.563277e-06
10.6 7.362584e-06
10.65 7.168123e-06
10.7 6.979673e-06
10.75 6.797022e-06
10.8 6.619965e-06
10.85 6.448306e-06
10.9 6.281858e-06
10.95 6.120438e-06
11 5.963873e-06
11.05 5.811997e-06
11.1 5.664648e-06
11.15 5.521671e-06
11.2 5.38292e-06
11.25 5.248249e-06
11.3 5.117523e-06
11.35 4.990609e-06
11.4 4.86738e-06
11.45 4.747712e-06
11.5 4.63149e-06
11.55 4.518598e-06
11.6 4.408928e-06
11.65 4.302374e-06
11.7 4.198835e-06
11.75 4.098214e-06
11.8 4.000416e-06
11.85 3.905351e-06
11.9 3.81293e-06
11.95 3.723071e-06
12 3.635692e-06
12.05 3.550714e-06
12.1 3.468062e-06
12.15 3.387662e-06
12.2 3.309446e-06
12.25 3.233344e-06
12.3 3.159292e-06
12.35 3.087225e-06
12.4 3.017084e-06
12.45 2.94881e-06
12.5 2.882344e-06
12.55 2.817633e-06
12.6 2.754624e-06
12.65 2.693265e-06
12.7 2.633507e-06
12.75 2.575301e-06
12.8 2.518603e-06
12.85 2.463366e-06
12.9 2.409549e-06
12.95 2.357108e-06
13 2.306005e-06
13.05 2.256199e-06
13.1 2.207653e-06
13.15 2.160331e-06
13.2 2.114197e-06
13.25 2.069217e-06
13.3 2.025358e-06
13.35 1.982588e-06
13.4 1.940877e-06
13.45 1.900193e-06
13.5 1.860508e-06
13.55 1.821794e-06
13.6 1.784024e-06
13.65 1.747171e-06
13.7 1.71121e-06
13.75 1.676117e-06
13.8 1.641866e-06
13.85 1.608436e-06
13.9 1.575803e-06
13.95 1.543945e-06
14 1.512843e-06
14.05 1.482474e-06
14.1 1.45282e-06
14.15 1.42386e-06
14.2 1.395577e-06
14.25 1.367953e-06
14.3 1.340969e-06
14.35 1.314608e-06
14.4 1.288855e-06
14.45 1.263693e-06
14.5 1.239107e-06
14.55 1.215081e-06
14.6 1.191601e-06
14.65 1.168653e-06
14.7 1.146223e-06
14.75 1.124297e-06
14.8 1.102862e-06
14.85 1.081907e-06
14.9 1.061418e-06
14.95 1.041384e-06
15 1.021793e-06
15.05 1.002634e-06
15.1 9.838958e-07
15.15 9.655682e-07
15.2 9.476406e-07
15.25 9.301032e-07
15.3 9.129461e-07
15.35 8.9616e-07
15.4 8.797356e-07
15.45 8.636639e-07
15.5 8.479365e-07
15.55 8.325446e-07
15.6 8.174803e-07
15.65 8.027354e-07
15.7 7.883023e-07
15.75 7.741733e-07
15.8 7.603411e-07
15.85 7.467987e-07
15.9 7.335389e-07
15.95 7.205551e-07
16 7.078407e-07
16.05 6.953893e-07
16.1 6.831946e-07
16.15 6.712506e-07
16.2 6.595513e-07
16.25 6.480911e-07
16.3 6.368643e-07
16.35 6.258655e-07
16.4 6.150893e-07
16.45 6.045307e-07
16.5 5.941845e-07
16.55 5.840459e-07
16.6 5.741101e-07
16.65 5.643725e-07
16.7 5.548284e-07
16.75 5.454736e-07
16.8 5.363037e-07
16.85 5.273145e-07
16.9 5.18502e-07
16.95 5.098621e-07
17 5.01391e-07
17.05 4.930849e-07
17.1 4.849401e-07
17.15 4.769531e-07
17.2 4.691203e-07
17.25 4.614383e-07
17.3 4.539037e-07
17.35 4.465135e-07
17.4 4.392643e-07
17.45 4.321531e-07
17.5 4.251768e-07
17.55 4.183326e-07
17.6 4.116176e-07
17.65 4.05029e-07
17.7 3.98564e-07
17.75 3.9222e-07
17.8 3.859944e-07
17.85 3.798847e-07
17.9 3.738884e-07
17.95 3.68003e-07
18 3.622263e-07
18.05 3.565559e-07
18.1 3.509896e-07
18.15 3.455252e-07
18.2 3.401606e-07
18.25 3.348936e-07
18.3 3.297222e-07
18.35 3.246445e-07
18.4 3.196585e-07
18.45 3.147623e-07
18.5 3.09954e-07
18.55 3.052318e-07
18.6 3.00594e-07
18.65 2.960389e-07
18.7 2.915647e-07
18.75 2.871698e-07
18.8 2.828526e-07
18.85 2.786115e-07
18.9 2.74445e-07
18.95 2.703515e-07
19 2.663297e-07
19.05 2.62378e-07
19.1 2.58495e-07
19.15 2.546795e-07
19.2 2.5093e-07
19.25 2.472453e-07
19.3 2.43624e-07
19.35 2.400649e-07
19.4 2.365668e-07
19.45 2.331285e-07
19.5 2.297487e-07
19.55 2.264265e-07
19.6 2.231606e-07
19.65 2.199499e-07
19.7 2.167934e-07
19.75 2.136901e-07
19.8 2.106388e-07
19.85 2.076387e-07
19.9 2.046886e-07
19.95 2.017877e-07
20 1.989351e-07
20.05 1.961297e-07
20.1 1.933708e-07
20.15 1.906573e-07
&
@target G0.S1
@type xy
1.245 1
1.78 0.27927608
2.76 0.037534321
2.98 0.025324145
3.28 0.014920453
3.792 0.007002272
4.8 0.001808158
6.6 0.000277471
10 2.31661e-05
15 1.48856e-06
20 1.82017e-07
&
@target G0.S2
@type xy
1.25 0.9799411
1.3 0.9438045
1.35 0.9102905
1.4 0.8791219
1.45 0.8500593
1.5 0.8228949
1.55 0.7974473
1.6 0.7735579
1.65 0.7510869
1.7 0.7299107
1.75 0.7099199
1.8 0.691017
1.85 0.673115
1.9 0.6561359
1.95 0.6400098
2 0.6246734
2.05 0.6100699
2.1 0.5961475
2.15 0.5828593
2.2 0.5701628
2.25 0.5580189
2.3 0.5463922
2.35 0.5352501
2.4 0.5245627
2.45 0.5143025
2.5 0.5044443
2.55 0.4949648
2.6 0.4858423
2.65 0.477057
2.7 0.4685903
2.75 0.4604252
2.8 0.4525456
2.85 0.4449369
2.9 0.4375851
2.95 0.4304773
3 0.4236016
3.05 0.4169467
3.1 0.410502
3.15 0.4042577
3.2 0.3982044
3.25 0.3923336
3.3 0.386637
3.35 0.3811069
3.4 0.3757361
3.45 0.3705178
3.5 0.3654455
3.55 0.3605131
3.6 0.3557148
3.65 0.3510453
3.7 0.3464994
3.75 0.3420722
3.8 0.3377591
3.85 0.3335557
3.9 0.3294579
3.95 0.3254616
4 0.3215632
4.05 0.317759
4.1 0.3140457
4.15 0.31042
4.2 0.3068789
4.25 0.3034193
4.3 0.3000385
4.35 0.2967338
4.4 0.2935027
4.45 0.2903427
4.5 0.2872514
4.55 0.2842267
4.6 0.2812664
4.65 0.2783683
4.7 0.2755307
4.75 0.2727516
4.8 0.2700292
4.85 0.2673617
4.9 0.2647475
4.95 0.2621851
5 0.2596728
5.05 0.2572093
5.1 0.254793
5.15 0.2524227
5.2 0.2500971
5.25 0.2478148
5.3 0.2455746
5.35 0.2433755
5.4 0.2412162
5.45 0.2390958
5.5 0.2370131
5.55 0.2349671
5.6 0.2329569
5.65 0.2309816
5.7 0.2290402
5.75 0.2271318
5.8 0.2252557
5.85 0.223411
5.9 0.2215968
5.95 0.2198126
6 0.2180574
6.05 0.2163307
6.1 0.2146317
6.15 0.2129597
6.2 0.2113141
6.25 0.2096943
6.3 0.2080997
6.35 0.2065297
6.4 0.2049837
6.45 0.2034612
6.5 0.2019616
6.55 0.2004844
6.6 0.1990292
6.65 0.1975953
6.7 0.1961824
6.75 0.19479
6.8 0.1934177
6.85 0.192065
6.9 0.1907315
6.95 0.1894167
7 0.1881204
7.05 0.186842
7.1 0.1855813
7.15 0.1843379
7.2 0.1831113
7.25 0.1819014
7.3 0.1807076
7.35 0.1795298
7.4 0.1783675
7.45 0.1772205
7.5 0.1760885
7.55 0.1749712
7.6 0.1738683
7.65 0.1727795
7.7 0.1717045
7.75 0.1706431
7.8 0.169595
7.85 0.16856
7.9 0.1675379
7.95 0.1665283
8 0.1655311
8.05 0.164546
8.1 0.1635728
8.15 0.1626113
8.2 0.1616613
8.25 0.1607226
8.3 0.1597949
8.35 0.1588781
8.4 0.157972
8.45 0.1570764
8.5 0.1561912
8.55 0.155316
8.6 0.1544508
8.65 0.1535954
8.7 0.1527497
8.75 0.1519134
8.8 0.1510864
8.85 0.1502686
8.9 0.1494597
8.95 0.1486597
9 0.1478684
9.05 0.1470857
9.1 0.1463114
9.15 0.1455454
9.2 0.1447875
9.25 0.1440376
9.3 0.1432957
9.35 0.1425615
9.4 0.141835
9.45 0.141116
9.5 0.1404044
9.55 0.1397
9.6 0.1390029
9.65 0.1383129
9.7 0.1376298
9.75 0.1369536
9.8 0.1362841
9.85 0.1356213
9.9 0.134965
9.95 0.1343152
10 0.1336718
10.05 0.1330346
10.1 0.1324036
10.15 0.1317787
10.2 0.1311598
10.25 0.1305468
10.3 0.1299397
10.35 0.1293382
10.4 0.1287425
10.45 0.1281523
10.5 0.1275676
10.55 0.1269884
10.6 0.1264145
10.65 0.1258458
10.7 0.1252824
10.75 0.1247241
10.8 0.1241709
10.85 0.1236227
10.9 0.1230794
10.95 0.1225409
11 0.1220072
11.05 0.1214783
11.1 0.120954
11.15 0.1204344
11.2 0.1199193
11.25 0.1194086
11.3 0.1189024
11.35 0.1184006
11.4 0.117903
11.45 0.1174097
11.5 0.1169207
11.55 0.1164357
11.6 0.1159549
11.65 0.1154781
11.7 0.1150053
11.75 0.1145364
11.8 0.1140714
11.85 0.1136103
11.9 0.1131529
11.95 0.1126993
12 0.1122494
12.05 0.1118032
12.1 0.1113606
12.15 0.1109215
12.2 0.110486
12.25 0.1100539
12.3 0.1096253
12.35 0.1092
12.4 0.1087782
12.45 0.1083596
12.5 0.1079444
12.55 0.1075323
12.6 0.1071235
12.65 0.1067178
12.7 0.1063153
12.75 0.1059159
12.8 0.1055195
12.85 0.1051261
12.9 0.1047357
12.95 0.1043483
13 0.1039638
13.05 0.1035821
13.1 0.1032034
13.15 0.1028274
13.2 0.1024542
13.25 0.1020838
13.3 0.1017161
13.35 0.1013512
13.4 0.1009888
13.45 0.1006292
13.5 0.1002721
13.55 0.09991759
13.6 0.09956564
13.65 0.09921623
13.7 0.0988693
13.75 0.09852485
13.8 0.09818285
13.85 0.09784326
13.9 0.09750606
13.95 0.09717123
14 0.09683874
14.05 0.09650857
14.1 0.09618069
14.15 0.09585507
14.2 0.09553171
14.25 0.09521056
14.3 0.09489162
14.35 0.09457485
14.4 0.09426023
14.45 0.09394775
14.5 0.09363738
14.55 0.09332909
14.6 0.09302287
14.65 0.0927187
14.7 0.09241655
14.75 0.09211641
14.8 0.09181826
14.85 0.09152207
14.9 0.09122783
14.95 0.09093551
15 0.0906451
15.05 0.09035659
15.1 0.09006994
15.15 0.08978514
15.2 0.08950218
15.25 0.08922104
15.3 0.08894169
15.35 0.08866413
15.4 0.08838833
15.45 0.08811428
15.5 0.08784196
15.55 0.08757135
15.6 0.08730245
15.65 0.08703522
15.7 0.08676966
15.75 0.08650576
15.8 0.08624348
15.85 0.08598283
15.9 0.08572378
15.95 0.08546633
16 0.08521045
16.05 0.08495613
16.1 0.08470335
16.15 0.08445211
16.2 0.08420239
16.25 0.08395417
16.3 0.08370744
16.35 0.08346219
16.4 0.0832184
16.45 0.08297607
16.5 0.08273517
16.55 0.0824957
16.6 0.08225764
16.65 0.08202098
16.7 0.0817857
16.75 0.08155181
16.8 0.08131927
16.85 0.08108809
16.9 0.08085825
16.95 0.08062973
17 0.08040253
17.05 0.08017663
17.1 0.07995203
17.15 0.07972871
17.2 0.07950666
17.25 0.07928587
17.3 0.07906634
17.35 0.07884804
17.4 0.07863096
17.45 0.07841511
17.5 0.07820046
17.55 0.07798702
17.6 0.07777475
17.65 0.07756367
17.7 0.07735375
17.75 0.07714499
17.8 0.07693738
17.85 0.07673091
17.9 0.07652557
17.95 0.07632135
18 0.07611824
18.05 0.07591623
18.1 0.07571531
18.15 0.07551548
18.2 0.07531672
18.25 0.07511903
18.3 0.07492239
18.35 0.07472681
18.4 0.07453226
18.45 0.07433875
18.5 0.07414626
18.55 0.07395479
18.6 0.07376433
18.65 0.07357486
18.7 0.07338639
18.75 0.0731989
18.8 0.07301239
18.85 0.07282685
18.9 0.07264226
18.95 0.07245864
19 0.07227595
19.05 0.07209421
19.1 0.0719134
19.15 0.07173351
19.2 0.07155454
19.25 0.07137648
19.3 0.07119933
19.35 0.07102307
19.4 0.07084769
19.45 0.07067321
19.5 0.0704996
19.55 0.07032685
19.6 0.07015497
19.65 0.06998395
19.7 0.06981378
19.75 0.06964445
19.8 0.06947596
19.85 0.06930829
19.9 0.06914146
19.95 0.06897544
20 0.06881024
20.05 0.06864584
20.1 0.06848224
20.15 0.06831944
&
@target G0.S3
@type xy
1.245 1
1.78 0.69959688
2.76 0.45842968
2.98 0.42529072
3.28 0.38703307
3.792 0.3364574
4.8 0.26740707
6.6 0.19724084
10 0.13332951
15 0.091123603
20 0.0696844
&


==> plots/plot_comparison <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Fri Apr 12 15:58:48 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -0.05, 110, 1.1
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "R\sdot\N (\cE\C)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 10
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Property ratio (X/X\s0\N)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place normal
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.85, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 2
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "plot_comparison"
@    s0 legend  "E\sBE\N"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 2
@    s1 symbol size 1.000000
@    s1 symbol color 2
@    s1 symbol pattern 1
@    s1 symbol fill color 2
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 2
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 2
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "plot_comparison"
@    s1 legend  "P\seh\N"
@target G0.S0
@type xy
13.8 1
14.9 0.927712
16.4 0.84425831
18.96 0.73393459
24 0.58331099
25 0.56224537
33 0.4302532
50 0.29083962
75 0.19877335
100 0.15200674
&
@target G0.S1
@type xy
13.8 1
14.9 0.67469304
16.4 0.39751492
18.96 0.18655651
24 0.048173445
25 0.041690844
33 0.007392465
50 0.000617198
75 3.96588e-05
100 4.84935e-06
&


==> plots/plot_log_log_be <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Tue Apr 30 16:12:45 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -2, 1.1, 0
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "Log R\sdot\N (nm)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Log Binding Energy (eV)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.5
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place normal
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.75, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 2
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "plot_log_log_be"
@    s0 legend  "XCHF method (this work)"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 4
@    s1 symbol size 1.000000
@    s1 symbol color 2
@    s1 symbol pattern 1
@    s1 symbol fill color 2
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 2
@    s1 line pattern 0
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 2
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "plot_log_log_be"
@    s1 legend  "Pseudopotential+CI"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 3
@    s2 symbol size 1.000000
@    s2 symbol color 3
@    s2 symbol pattern 0
@    s2 symbol fill color 4
@    s2 symbol fill pattern 1
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 1
@    s2 line linewidth 1.0
@    s2 line color 3
@    s2 line pattern 0
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 3
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "plot_log_log_be"
@    s2 legend  "Experiment"
@target G0.S0
@type xy
0.432696027     -0.36663095
0.471494113     -0.40822422
0.508682744     -0.45943754
0.574850112     -0.53718579
0.680078202     -0.66178689
0.81847801      -0.82573414
0.999451662     -1.0332682
1.175834193     -1.2329617
1.300996023     -1.3702562
&
@target G0.S1
@type xy
0.68124 -0.73798105
0.51587 -0.53228093
&
@target G0.S2
@type xy
0.57978 -0.56384054
&


==> plots/plot_log_log_be_comp_ddot <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Wed May 22 14:04:23 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0.4, -2, 1.4, 0
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "Log D\sdot\N(nm)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.5
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Log Binding Energy (eV)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.5
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place normal
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.6, 0.83
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 2
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "plot_log_log_be_comp_ddot"
@    s0 legend  "XCHF method (this work)"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 1
@    s1 symbol size 1.000000
@    s1 symbol color 2
@    s1 symbol pattern 1
@    s1 symbol fill color 2
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 50
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 2
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 2
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "plot_log_log_be_comp_ddot"
@    s1 legend  "Franceschetti and Zunger extrapolation"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 3
@    s2 symbol size 1.000000
@    s2 symbol color 3
@    s2 symbol pattern 1
@    s2 symbol fill color 3
@    s2 symbol fill pattern 1
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 1
@    s2 line linewidth 1.0
@    s2 line color 3
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 3
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "plot_log_log_be_comp_ddot"
@    s2 legend  "Jasieniak et al. "
@    s3 hidden false
@    s3 type xy
@    s3 symbol 8
@    s3 symbol size 1.000000
@    s3 symbol color 4
@    s3 symbol pattern 1
@    s3 symbol fill color 4
@    s3 symbol fill pattern 1
@    s3 symbol linewidth 10.5
@    s3 symbol linestyle 1
@    s3 symbol char 100
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 1
@    s3 line linestyle 1
@    s3 line linewidth 1.0
@    s3 line color 4
@    s3 line pattern 0
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 4
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "plot_log_log_be_comp_ddot"
@    s3 legend  "Meulenberg et al."
@    s4 hidden false
@    s4 type xy
@    s4 symbol 6
@    s4 symbol size 1.000000
@    s4 symbol color 12
@    s4 symbol pattern 1
@    s4 symbol fill color 12
@    s4 symbol fill pattern 1
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 100
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 1
@    s4 line linestyle 1
@    s4 line linewidth 1.0
@    s4 line color 12
@    s4 line pattern 0
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 12
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "plot_log_log_be_comp_ddot"
@    s4 legend  "Franceschetti and Zunger"
@target G0.S0
@type xy
0.44171153 -0.40455406
0.47421687 -0.43714089
0.51567168 -0.47807871
0.5789887 -0.5388967
0.68141499 -0.6386539
0.81954394 -0.77082995
1 -0.9409005
1.1760913 -1.1061959
1.30103 -1.2226912
&
@target G0.S1
@type xy
0.44171153 -0.41951317
0.47421687 -0.46293574
0.51567168 -0.51724473
0.5789887 -0.60056388
0.68141499 -0.7328342
0.81954394 -0.91313943
1 -1.1484
1.1760913 -1.3779702
1.30103 -1.5408528
&
@target G0.S2
@type xy
0.44171153 -0.30295715
0.47421687 -0.33568272
0.51567168 -0.37718023
0.5789887 -0.44196296
0.68141499 -0.54724938
0.81954394 -0.69480772
1 -0.89290353
1.1760913 -1.0909309
1.30103 -1.2336826
&
@target G0.S3
@type xy
0.5789887 -0.56384054
&
@target G0.S4
@type xy
0.51567168 -0.53228093
0.68141499 -0.73798105
&


==> plots/plot_log_log_be_comp_ddot_v2 <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Mon Jun  3 14:07:55 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0.3, -2, 1.4, 0
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "Log D\sdot\N(nm)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Log Binding Energy (eV)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.5
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place normal
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.6, 0.83
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 2
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "plot_log_log_be_comp_ddot"
@    s0 legend  "XCHF method (this work)"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 4
@    s1 symbol size 1.240000
@    s1 symbol color 2
@    s1 symbol pattern 1
@    s1 symbol fill color 2
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 50
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 0
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 2
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 2
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "plot_log_log_be_comp_ddot"
@    s1 legend  "Meulenberg et al."
@    s2 hidden false
@    s2 type xy
@    s2 symbol 3
@    s2 symbol size 1.000000
@    s2 symbol color 3
@    s2 symbol pattern 1
@    s2 symbol fill color 3
@    s2 symbol fill pattern 1
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 0
@    s2 line linestyle 1
@    s2 line linewidth 1.0
@    s2 line color 3
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 3
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "plot_log_log_be_comp_ddot"
@    s2 legend  "Franceschetti and Zunger "
@    s3 hidden false
@    s3 type xy
@    s3 symbol 1
@    s3 symbol size 0.090000
@    s3 symbol color 4
@    s3 symbol pattern 1
@    s3 symbol fill color 4
@    s3 symbol fill pattern 1
@    s3 symbol linewidth 10.5
@    s3 symbol linestyle 1
@    s3 symbol char 10
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 0
@    s3 line linestyle 1
@    s3 line linewidth 1.0
@    s3 line color 1
@    s3 line pattern 0
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 4
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "plot_log_log_be_comp_ddot"
@    s3 legend  "Jasieniak et al."
@target G0.S0
@type xy
0.44171153 -0.40455406
0.47421687 -0.43714089
0.51567168 -0.47807871
0.5789887 -0.5388967
0.68141499 -0.6386539
0.81954394 -0.77082995
1 -0.9409005
1.1760913 -1.1061959
1.30103 -1.2226912
&
@target G0.S1
@type xy
0.5789887 -0.56384054
&
@target G0.S2
@type xy
0.51567168 -0.53228093
0.68141499 -0.73798105
&
@target G0.S3
@type xy
0.40993312 -0.49485002
0.46089784 -0.55284197
0.50785587 -0.58502665
0.50785587 -0.58502665
0.60530505 -0.69897
0.60852603 -0.67778071
0.62221402 -0.69897
0.71096312 -0.79588002
0.75511227 -0.82390874
0.75511227 -0.82390874
0.75511227 -0.82390874
0.80482068 -0.88605665
0.80482068 -0.88605665
&


==> plots/plot_log_log_coul <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Tue Apr 30 16:16:06 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -0.5, 1.1, 0.41
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "Log R\sdot\N (nm)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Log Coulomb Energy (eV)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place normal
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.75, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 2
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "plot_log_log_coul"
@    s0 legend  "XCHF method (this work)"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 4
@    s1 symbol size 1.000000
@    s1 symbol color 2
@    s1 symbol pattern 1
@    s1 symbol fill color 2
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 2
@    s1 line pattern 0
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 2
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "plot_log_log_coul"
@    s1 legend  "Pseudopotential+CI"
@target G0.S0
@type xy
0.432696027     0.38844865
0.471494113     0.35612509
0.508682744     0.31600829
0.574850112     0.25412245
0.680078202     0.15339231
0.81847801      0.018945926
0.999451662     -0.1535561
1.175834193     -0.32281209
1.300996023     -0.44133783
&
@target G0.S1
@type xy
0.68124 0.17464119
0.51587 0.3174365
&


==> plots/plot_log_log_coul_ddot <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Thu Jun  6 22:36:11 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -0.5, 1.4, 0.8
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "Log [D\sdot\N / 1 nm]"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Log [A / 1 eV]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place normal
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.6, 0.82
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 2
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "plot_log_log_coul"
@    s0 legend  "eh-XCHF method (this work)"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 1
@    s1 symbol size 1.240000
@    s1 symbol color 12
@    s1 symbol pattern 1
@    s1 symbol fill color 12
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 0
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 2
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 12
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "plot_log_log_coul"
@    s1 legend  "Franceschetti and Zunger "
@target G0.S0
@type xy
0.095203336 0.7265649
0.25328409 0.57141277
0.43269603 0.387838
0.47149411 0.355251
0.50868274 0.314313
0.57485011 0.253495
0.6800782 0.153738
0.81847801 0.021562
0.99945166 -0.14851
1.1758342 -0.3138
1.300996 -0.4303
&
@target G0.S1
@type xy
0.25527251 0.54444014
0.68124 0.17464119
0.51587 0.3174365
&


==> plots/plot_log_log_recomb <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Thu Jun  6 22:40:39 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -21.5, 1.34, -13.5
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "Log [D\sdot\N / 1 nm]"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Log Recombination Probability"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 1
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place normal
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.7, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 1
@    s0 symbol size 1.000000
@    s0 symbol color 2
@    s0 symbol pattern 1
@    s0 symbol fill color 2
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 0
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 2
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "plot_log_log_recomb"
@    s0 legend  "eh-XCHF method"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 0
@    s1 symbol size 1.000000
@    s1 symbol color 1
@    s1 symbol pattern 1
@    s1 symbol fill color 1
@    s1 symbol fill pattern 0
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 1
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 1
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "plot_log_log_recomb_ddot"
@    s1 legend  ""
@target G0.S0
@type xy
0.076268392 -14.139786
0.22792324 -14.693646
0.43269603 -15.565232
0.47149411 -15.736126
0.50868274 -15.965878
0.57485011 -16.294421
0.6800782 -16.882424
0.81847801 -17.696442
0.99945166 -18.774807
1.1758342 -19.966893
1.300996 -20.879548
&
@target G0.S1
@type xy
0.076268392 -13.697325
0.22792324 -14.545045
0.43269603 -15.689684
0.47149411 -15.906558
0.50868274 -16.114435
0.57485011 -16.484297
0.6800782 -17.072501
0.81847801 -17.846128
0.99945166 -18.857735
1.1758342 -19.843678
1.300996 -20.543307
&


==> plots/plot_log_recomb <==
# Grace project file
#
@version 50122
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 14 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 15 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 16 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 17 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 18 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 19 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 20 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 21 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 22 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 23 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 24 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 25 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 26 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 27 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 28 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 29 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 31 to "Symbol-Regular", "Symbol-Regular"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 36 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 37 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 38 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 39 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 40 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 41 to "URWGothicL-Book", "URWGothicL-Book"
@map font 42 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 43 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 44 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 45 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 46 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 47 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 48 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Fri Apr 12 15:55:00 2013"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -22, 0.1, -14
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.150000, 0.850000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "1/r\sdot\N (\cE\C)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.05
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Log recombination probability"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 1
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.7, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 2
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "plot_log_recomb"
@    s0 legend  "Explicitly correlated method"
@target G0.S0
@type xy
0.07233 -15.565232
0.067114 -15.736126
0.061004 -15.965878
0.052728 -16.294421
0.04165 -16.882424
0.04 -16.945191
0.03030303 -17.696442
0.02 -18.774807
0.013333 -19.966893
0.01 -20.879548
&


==> sections/sec_dielec.tex <==
\subsection{Effect of dielectric constant}
\label{sec:dielec}
The dielectric function directly impacts the electron-hole 
interaction term and is important for computation of accurate exciton binding energies. 
Earlier studies have demonstrated the importance of including size-dependent dielectric 
function for accurate calculation of exciton energy. We denote the general
size-dependent dielectric function as $\epsilon(\mathbf{r}_\mathrm{e},\mathbf{r}_\mathrm{h},D)$
where $D$ is the diameter of the dot. Although this expression is very accurate, it is 
computationally expensive to use because of its dependence on the electron and hole coordinates. 
Wang and Zunger have shown ~\cite{PhysRevB.53.9579} that accurate size-dependent dielectric constant can be obtained 
from $\epsilon(\mathbf{r}_\mathrm{e},\mathbf{r}_\mathrm{h},D)$ by performing integration 
using electron and hole densities as shown below
\begin{align}
	\epsilon(D) 
	&= \langle \epsilon(\mathbf{r}_\mathrm{e},\mathbf{r}_\mathrm{h},D) 
		\rho_\mathrm{e} \rho_\mathrm{h} \rangle .
\end{align}
The Wang-Zunger (WZ) expression for the dielectric constant is given by the following 
equation
\begin{align}
	{\epsilon}^{-1}_\mathrm{WZ}(D)
	&=
	\tilde{\epsilon}^{-1}_\infty(D) \\ \notag
	&-\beta_{\rho_\mathrm{e},\rho_\mathrm{h}}(D)
	\left[ 
		\tilde{\epsilon}^{-1}_\infty
		- (\tilde{\epsilon}_\infty + \Delta \epsilon_\mathrm{ion})^{-1}
	\right]
\end{align}
where the definition of the terms in the above expression can be found in Ref. \citenum{PhysRevB.53.9579}.
The above procedure for obtaining the size-dependent dielectric constant has been shown to accurately 
represent electron-hole interaction in quantum dots \cite{rabani:5355,PhysRevB.53.9579},
and was used for determining the dielectric constants for all the dots
listed in \ref{tab:cluster_tab}. 
\begin{table}
 \begin{center} 
  \caption{Exciton binding energy calculated using the XCHF method for both bulk CdSe dielectric constant($\epsilon_{6.2}$) and size dependent 
           dielectric constant procured from method given by Wang and Zunger($\epsilon_\mathrm{WZ}$).}
   \label{tab:comp_tab} 
    \begin{tabular}{ c c c } 
     $\mathrm{D_{dot}}$(nm) & $E_\mathrm{{BE}}(\epsilon_{\mathrm{WZ}})$  & $E_\mathrm{{BE}}(\epsilon_{6.2})$ \\ 
     \hline 
      2.71         & 0.429             & 0.394            \\
      2.96         & 0.391             & 0.365            \\
      3.23         & 0.347             & 0.333            \\
      3.76         & 0.290             & 0.289            \\

    \end{tabular}
  \end{center} 
\end{table} 


==> sections/sec_eq_table.tex <==
\begin{table}
 \begin{center} 
  \caption{Summary of functional forms of the scaling of the properties associated with exciton dissociation in CdSe quantum dots with respect to dot diameter}
   \label{tab:func_tab} 
    \begin{tabular}{ l c } 
     Property  &      Functional form  \\ 
     \hline 
      $\mathrm{log} A$              & $-0.9515(\mathrm{log D}) + 0.8047$     \\
      $\mathrm{log} E_\mathrm{{BE}}$         & $-0.9515(\mathrm{log D}) + 0.0123$     \\
      $\mathrm{log} P_\mathrm{{eh}}$         &     $ -6.1131(\mathrm{log D}) - 12.873$     \\
    \end{tabular}
  \end{center} 
\end{table} 


With respect to changing size of quantum dot, the properties of exciton dissociation can be quantified through the functional forms found in \ref{tab:func_tab}. In general
the properties scale as $A(\mathrm{log D} + B$. For both binding energy and Coulomb energy the scaling is shown to be sublinear which corresponds to previous findings by both 
Wang and Zunger and Meulenberg et al. However, recombination probability, having a much larger $ A $ and $B$ value is shown to decrease at a faster rate than that found in binding energy
and Coulomb energy. 


==> temp1.tex <==
%\subsection*{Recombination probability} 
The central quantity of interest for the present work 
is the electron-hole pair density $\rho(\mathbf{r}_\mathrm{e},\mathbf{r}_\mathrm{h})$
which is the probability density of finding an electron and a hole in the 
neighborhood  of
$\mathbf{r}_\mathrm{e}$ and $\mathbf{r}_\mathrm{h}$. respectively. 
The electron-hole pair density for a quantum contain detailed
information about the spatial distribution of the quasi-particle in the quantum dot.
The pair density is mathematically complicated quantity and is
generally obtained from an underlying wavefunction. Direct construction 
of the pair-density is also possible as long as $N-\mathrm{representability}$
can be satisfied. 
For an interacting electron-hole system, the pair density 
is not equal to the product of electron and hole densities
\begin{align}
	\rho_\mathrm{eh}(\mathbf{r}_\mathrm{e},\mathbf{r}_\mathrm{h})
	\neq
	\rho_\mathrm{e}(\mathbf{r}_\mathrm{e})
	\rho_\mathrm{h}(\mathbf{r}_\mathrm{h}) .
\end{align} 
Both electron-hole recombination probability and exciton binding energy can be
computed directly from the pair density. The electron-hole recombination 
probability $P_\mathrm{eh}$ is related to the pair density as
\begin{align}
\label{eq:peh}
	P_\mathrm{eh} 
	&=
	\frac{1}{N_\mathrm{e}N_\mathrm{h}}
	\int d\mathbf{r}_\mathrm{e}
	\int_{\mathbf{r}_\mathrm{e}-\frac{\Delta}{2}}^{\mathbf{r}_\mathrm{e}+\frac{\Delta}{2}} 
	d\mathbf{r}_\mathrm{h} \,\,
	\rho_\mathrm{eh}(\mathbf{r}_\mathrm{e},\mathbf{r}_\mathrm{h}).
\end{align}
In the above equation, $P_\mathrm{eh}$ is the probability of finding a hole 
in a cube of volume $\Delta^3$ centered at the electron position. 
Knowledge of the electron-hole pair density allow us compute the 
exciton binding energy using the following expression
\begin{align}
\label{eq:eb}
 E_\mathrm{BE}
 &=
 \int d\mathbf{r}_\mathrm{e} d\mathbf{r}_\mathrm{h} \,\,
 \rho_\mathrm{eh}(\mathbf{r}_\mathrm{e},\mathbf{r}_\mathrm{h})
 r^{-1}_\mathrm{eh} \epsilon^{-1}(\mathbf{r}_\mathrm{e},\mathbf{r}_\mathrm{h}).
\end{align}
In the following calculations, the electron-hole pair
density was computed from a variationally optimized electron-hole wavefunction 
and the details of the calculations are presented in the Method section.
The exciton binding energy were computed for  series of CdSe clusters ranging from 
$\mathrm{Cd}_{199}\mathrm{Se}_{195}$ to $\mathrm{Cd}_{74608}\mathrm{Se}_{74837}$.
The approximate diameter of these quantum dots are in the range of  
$3$ to $20\mathrm{nm}$, respectively and the results are presented in 
Table \ref{tab:cluster_tab}.
\begin{table}
  \begin{center}
   \caption{\textbf{Radius of CdSe particle versus actual cluster size and corresponding binding energy. All binding energies
                    given are calculated using the XCCI method.}}
   \note[Ari]{Three significant figures for column 3}
   \label{tab:cluster_tab}
    \begin{tabular}{l l l}
      $R_\mathrm{dot}$ (nm) & $\mathrm{Cd}_{x}\mathrm{Se}_{y}$   &  $E_\mathrm{BE}$(eV)  \\
      \hline
      1.38                & $\mathrm{Cd}_{199}\mathrm{Se}_{195}$             & 0.39350 \\ 
      1.49                & $\mathrm{Cd}_{232}\mathrm{Se}_{257}$             & 0.36548 \\ 
      1.64                & $\mathrm{Cd}_{311}\mathrm{Se}_{352}$             & 0.33260  \\
%      1.66                & Ref. \citenum{PhysRevLett.78.915}    &  0.294 \\
      1.90                & $\mathrm{Cd}_{513}\mathrm{Se}_{515}$             & 0.28913  \\
%      ZZZ                 & Ref. \citenum{doi:10.1021/nn8006916}  &   ZZZ \\
      2.41                & $\mathrm{Cd}_{1012}\mathrm{Se}_{1063}$           & 0.22980 \\ 
%      2.43                & Ref. \citenum{PhysRevLett.78.915}  &    0.184 \\
      2.50                & $\mathrm{Cd}_{1159}\mathrm{Se}_{1183}$           & 0.22150 \\ 
      3.30                & $\mathrm{Cd}_{2704}\mathrm{Se}_{2661}$           & 0.16950 \\ 
      5.00                & $\mathrm{Cd}_{9338}\mathrm{Se}_{9363}$           & 0.11458 \\ 
      7.50                & $\mathrm{Cd}_{31534}\mathrm{Se}_{31509}$         & 0.07831 \\ 
      10.0                & $\mathrm{Cd}_{74608}\mathrm{Se}_{74837}$         & 0.05988
    \end{tabular}
  \end{center}  
\end{table}   
As expected, it is seen that binding energy decreases as the size of the quantum dot increases.
This trend is in agreement with earlier results of effect of dot size on binding energy. 
For comparison we have also listed theoretical and experimental binding energies from 
earlier studies. For $R_\mathrm{dot}$ equal to $1.66$ and $2.41\mathrm{nm}$, 
Franceschetti and  Zunger have computed highly accurate binding energies using pseudopotential based 
configuration interaction method.\cite{PhysRevLett.78.915}. Meulenberg and coworkers ~\cite{doi:10.1021/nn8006916} have obtained experimental excition binding energy
for CdSe quantum dots and their result for ZZZ nm is included in Table \ref{tab:cluster_tab}
The computed exciton binding energies were found to be in good agreement with
previous results and are presented in  in Fig. ZZZ. It was found that the computed exciton binding energies scales as $R_\mathrm{dot}^{-n}$ with  $n=ZZZ$. This is comparable to the experimental and configuration interaction results
of $n=ZZZ$ and ZZZ, respectively. Another importance quantity that is directly related to the
electron-hole interaction is the electron-hole Coulomb energy. We have used the definition by 
Franceschetti and  Zunger and defined the electron-hole Coulomb energy as the product of 
exciton binding energy with 
\begin{align}
\label{eq:eb}
 A
 &=
 \int d\mathbf{r}_\mathrm{e} d\mathbf{r}_\mathrm{h} \,\,
 \rho_\mathrm{eh}(\mathbf{r}_\mathrm{e},\mathbf{r}_\mathrm{h})
 r^{-1}_\mathrm{eh} .
\end{align}
If the dielectric function is independent of position, then the electron-hole Coulomb energy
can be obtained by multiplying the binding energy by the dielectric constant $A=\epsilon E_\mathrm{EB}$.
In Fig. ZZZ, we have compared the electron-hole Coulomb energy with the pseudopotential+CI calculations
by Franceschetti and  Zunger and the results were found to be in good agreement with each other. 
\par 
In addition to binding energy, electron-hole recombination probability was calculated for the same size range of 
quantum dot. 
Studying recombination probability is essential due to the inherent information
associated with electron-hole recombination, including relation to lifetime measurements and efficiency of quantum dots for application 
various materials. It will be advantageous to have a prediction of how the recombination will change as a function of dot size. 
As described in Eq. \eqref{eq:peh}, the electron-hole pair density was 
also used in the computation of electron-hole recombination probabilities and the 
results are presented in Fig. ZZZ. A log-log plot of the $P_\mathrm{eh}$ versus 
$R_\mathrm{dot}$ indicates that the recombination probability also follows $R_\mathrm{dot}^{-n}$
dependence with $n=ZZZ$. One of the key results from this study is that the
electron-hole recombination probability decreases much faster that the exciton-binding energy with increasing dot
size. This is illustrated in Fig. \ref{fig:fig_comp_prop}, where comparison of the relative binding energy and recombination probability is presented with respect to dot size. It was found that for a ZZZ change in the dot radius, the exciton binding energy
and the recombination probability decreases by a factor of ZZZ and ZZZ, respectively. 
With respect to CdSe quantum dots, recombination as a function of the inverse of the dot size has not been well studied. However, in this work we compute 
recombination probability as a function of increasing dot size using the explicitly correlated method. 
The results are presented in ~\ref{fig:fig_recomb_prob_rdot} and ~\ref{fig:fig_log_recomb}. In general, as the size of the quantum dot 
increases, the exciton recombination probability decreases which is the trend that is expected due to the structure of the quantum dot system. This trend can 
be seen in ~\ref{fig:fig_recomb_prob_rdot}. Recombination probability can also be studied as a function of the inverse of rdot.
This can be seen in figure \ref{fig:fig_log_recomb}, where the log of recombination probability is plotted versus inverse of $r_\mathrm{dot}$.
The log of recombination is chosen here so as to emphasize the orders of magnitude change that can be observed for the range of dot size studied. 
Over the range of dot sizes studied, a five order of magnitude change is observed in the electron-hole recombination. 
\begin{figure}[ht] 
\begin{center} 
\includegraphics[width=100mm]{plots_new_res/plot_comparison.pdf}
\caption{Comparison of $E_{BE}$ and $P_{eh}$ relative properties versus $r_\mathrm{dot}$. }
\note[Ari] {
	[1]. Everything should be in "nm" \newline
	[2]. Remove one of the "double-points" from the plot and all tables \newline
	[3]. Use different symbols for Eb and Peh
}
\label{fig:fig_comp_prop}
\end{center}
\end{figure}
Therefore, from this data we can determine how recombination
probability will change as the size of the dot changes which is a quantity which has not been reported previously.
The recombination probability is heavily dependent on the form of the wavefunction. 
When the electron and hole recombine, they will be found at these small interparticle distances so therefore 
the wavefunction must be very accurate in order to be able to calculate recombination probability. 
The explicitly correlated method provides two components, the mean field component which describes
the long range electron-hole interaction and the explicit interparticle distance which describes the small range very efficiently. 


%As a step towards understanding the interaction between electron and hole, 
%the total exciton binding energy ($E_{\textrm{BE}}$) was calculated for a CdSe quantum dot
%system using the explicitly correlated configuration interaction method which is described in detail in the Methods 
%section. 
%Binding energy relies heavily on interaction 
%between the electron and hole, as it is a measure of the energy it takes to separate and electron and hole.
%It is known from previous benchmark calculation that explicitly correlated methods
%provides an accurate description of the
%%wavefunction at these small distances ~\cite{elward:124105,Elward2012182}.
%Therefore, the XCCI method was used to calculate $E_{\textrm{BE}}$ for a range of CdSe quantum dots. 



